Wi-Fi Channel Saturation as a Mechanism to Improve Passive Capture of Bluetooth Through Channel Usage Restriction

Bluetooth is a short-range wireless technology that provides audio and data links between personal smartphones and playback devices, such as speakers, headsets and car entertainment systems. Since its introduction in 2001, security researchers have suggested that the protocol is weak, and prone to a variety of attacks against its authentication, link management and encryption schemes. Key researchers in the field have suggested that reliable passive sniffing of Bluetooth traffic would enable the practical application of a range of currently hypothesised attacks. Restricting Bluetooth's frequency hopping behaviour by manipulation of the available channels, in order to make brute force attacks more effective has been a frequently proposed avenue of future research from the literature. This paper has evaluated the proposed approach in a series of experiments using the software defined radio tools and custom hardware developed by the Ubertooth project. The work concludes that the mechanism suggested by previous researchers may not deliver the proposed improvements, but describes an as yet undocumented interaction between Bluetooth and Wi-Fi technologies which may provide a Denial of Service attack mechanism.

==> papers.tex <==
References
Albazrqaoe, W. (2011). a Study of Bluetooth Frequency Hopping Sequence: Modeling and a Practical Attack. Michigan State University.
Albazrqaoe, W., Huang, J., \& Xing, G. (2016). Practical Bluetooth Traffic Sniffing : Systems and Privacy Implications. In MobiSys 16 Proceedings of the 14th Annual International Conference on Mobile Systems, Applications, and Services (pp. 333–345). Singapore: ACM. https://doi.org/10.1145/2906388.2906403

Bluetooth SIG. (2007). Bluetooth 2.1 (Core Specifications) (Vol. 2.1). Retrieved from https://www.bluetooth.com/specifications/adopted-specifications/legacy-specifications
Bluetooth SIG. (2013). Bluetooth 4.1 (Core Specifications) (Vol. 4.1). Retrieved from https://www.bluetooth.org/DocMan/handlers/DownloadDoc.ashx?doc_id=282159
Bluetooth SIG. (2016). Bluetooth 5.0 (Core Specifications) (Vol. 5.0). Retrieved from https://www.bluetooth.org/DocMan/handlers/DownloadDoc.ashx?doc_id=421043

Cheah, M., Shaikh, S. A., Haas, O., \& Ruddle, A. (2017). Towards a systematic security evaluation of the automotive Bluetooth interface. Vehicular Communications (Vol. 9). Elsevier Inc. https://doi.org/10.1016/j.vehcom.2017.02.008
Checkoway, S., Mccoy, D., Kantor, B., Anderson, D., Shacham, H., Savage, S., … Kohno, T. (2011). Comprehensive Experimental Analyses of Automotive Attack Surfaces. System, 6–6. Retrieved from http://www.usenix.org/events/security/tech/full_papers/Checkoway.pdf
Chen, L., Cooper, P., \& Liu, Q. (2012). Security in Bluetooth Networks and Communications. In L. Chen, J. Ji, \& Z. Zhang (Eds.), Wireless Network Security (pp. 77–94). Beijing: Springer.
Chernyshev, M., Valli, C., \& Johnstone, M. (2017). Revisiting Urban War Nibbling: Mobile Passive Discovery of Classic Bluetooth Devices Using Ubertooth One. IEEE Transactions on Information Forensics and Security, 12(7), 1625–1635. https://doi.org/10.1109/TIFS.2017.2678463
Chokshi, R. (2010). Yes! Wi-Fi and Bluetooth Can Coexist in Handheld Devices. Retrieved from http://www.marvell.com/wireless/assets/Marvell-WiFi-Bluetooth-Coexistence.pdf
CPU Benchmark. (2017). CPU Comparison. Retrieved from https://www.cpubenchmark.net/compare.php?cmp[]=3092\&cmp[]=1074
Dunning, J. P. (2010). Taming the blue beast: A survey of bluetooth based threats. IEEE Security and Privacy, 8(2), 20–27. https://doi.org/10.1109/MSP.2010.3
Gao, V. (2016). Debugging Bluetooth With An Android App. Retrieved May 26, 2017, from https://blog.bluetooth.com/debugging-bluetooth-with-an-android-app
Giousouf, A., \& Lemke, K. (2011). Bluetooth Security.
Gummadi, R., Wetherall, D., Greenstein, B., \& Seshan, S. (2007). Understanding and mitigating the impact of RF interference on 802.11 networks. ACM SIGCOMM Computer Communication Review, 37(4), 385. https://doi.org/10.1145/1282427.1282424
Haartsen, J. C. (2000). The Bluetooth Radio System. IEEE Personal Communications, (February), 28–36. Retrieved from http://citeseerx.ist.psu.edu/viewdoc/citations;jsessionid=EC2B8E030D8A95A43A4F0752A1100C74?doi=10.1.1.11.8115
Haataja, K., Hyppnen, K., Pasanen, S., \& Toivanen, P. (2013). Overview of Bluetooth Security. In Bluetooth Security Attacks: Comparative Analysis, Attacks, and Countermeasures (Vol. 2742, pp. 89–93). Springer. https://doi.org/10.1007/978-3-642-40646-1
Haines, B. (2010). Bluetooth Attacks. In Seven Deadliest Wireless Technologies Attacks (pp. 43–55). Elsevier. https://doi.org/10.1016/B978-1-59749-541-7.00003-5
Hassan, S. S., Bibon, S. Das, Hossain, M. S., \& Atiquzzaman, M. (2017). Security threats in Bluetooth technology. Computers and Security. https://doi.org/10.1016/j.cose.2017.03.008
Heffernan, D., \& Leen, G. (2001). Vehicles without wires. Computing \& Control Engineering Journal, 12(5), 205–211. https://doi.org/10.1049/cce:20010501
Hines, G. (2014). How to get to Windows CE Desktop. Retrieved November 25, 2017, from http://www.hyundai-forums.com/tucson-ix35-lm-models/304426-how-get-windows-ce-desktop.html
Hodgdon, C. (2003). Adaptive Frequency Hopping for Reduced Interference between Bluetooth and Wireless LAN. Retrieved September 8, 2017, from https://www.design-reuse.com/articles/5715/adaptive-frequency-hopping-for-reduced-interference-between-bluetooth-and-wireless-lan.html
Holtmann, M. (2014). Bringing the BlueZ back to Android. In Linux Foundation Android Builders Summit. San Jose. Retrieved from https://elinux.org/images/f/f5/Bringing_the_bluez_back_to_android--holtmann.pdf
Huang, J., Albazrqaoe, W., \& Xing, G. (2014). BlueID: A practical system for Bluetooth device identification. In Proceedings - IEEE INFOCOM (pp. 2849–2857). https://doi.org/10.1109/INFOCOM.2014.6848235
Jacobsson, M., \& Wetzel, S. (2001). Security Weaknesses in Bluetooth. In Topics in Cryptology - CT-RSA 2001 (pp. 176–191). San Francisco: Springer. Retrieved from https://link.springer.com/chapter/10.1007/3-540-45353-9_14
Muniz, J., \& Lakhani, A. (2013). Web Penetration Testing with Kali Linux.
Naggs, T. (2013). Ubertooth Mailing List. Retrieved November 8, 2017, from https://sourceforge.net/p/ubertooth/mailman/message/31237673/
Neumeier, R., \& Ostermayer, G. (2013). Analyzing coexistence issues in wireless radio networks: Simulation of Bluetooth interfered by multiple WLANs. Lecture Notes in Computer Science (Including Subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics), 8310 LNCS, 128–138. https://doi.org/10.1007/978-3-319-03871-1_12
Nusser, R., \& Pelz, R. M. (2000). Bluetooth-based wireless connectivity in an automotive environment. Vehicular Technology Conference Fall 2000. IEEE VTS Fall VTC2000. 52nd Vehicular Technology Conference (Cat. No.00CH37152), 4, 1935–1942. https://doi.org/10.1109/VETECF.2000.886152
O’Malley, J. (2017). Bluetooth Mesh Is Going To Be A Big Deal. Retrieved September 19, 2017, from http://www.gizmodo.co.uk/2017/07/bluetooth-mesh-is-going-to-be-a-big-deal-here-are-6-reasons-why-you-should-care/
Ossmann, M., \& Spill, D. (2009). Building an All-Channel Bluetooth Monitor. In ShmooCon 09 (p. 102).
Pelzl, J., \& Wollinger, T. (2006). Security Aspects of Mobile Communication Systems. In K. Lemke, C. Paar, \& M. Wolf (Eds.), Embedded Security in Cars (pp. 167–185). Berlin/Heidelberg: Springer-Verlag. https://doi.org/10.1007/3-540-28428-1
Popovski, P., Yomo, H., \& Prasad, R. (2006). Strategies for adaptive frequency hopping in the unlicensed bands. IEEE Wireless Communications, 13(6), 60–67. https://doi.org/10.1109/MWC.2006.275200
Rivertz, H. J. (2005). Bluetooth Security (Vol. DART/05/05). Oslo. Retrieved from papers3://publication/uuid/0f81fe0b-3210-4140-80f2-9cb6bfe8ae44
Ryan, M. (2013). Bluetooth: With Low Energy Comes Low Security. Proceedings of the 7th USENIX Conference on Offensive Technologies, 4. Retrieved from http://dl.acm.org/citation.cfm?id=2534748.2534754
Scarfone, K., Padgette, J., \& Chen, L. (2008). Guide to Bluetooth security. NIST Special Publication, 1(Guide to Bluetooth Security), 121. https://doi.org/10.6028/NIST.SP.800-121r1
Seri, B., \& Vishnepolsky, G. (2017). BlueBorne. Retrieved from http://go.armis.com/blueborne-technical-paper
Shaked, Y., \& Wool, A. (2005). Cracking the Bluetooth PIN. Proceedings of the 3rd International Conference on Mobile Systems, Applications, and Services - MobiSys ’05, 39–50. https://doi.org/10.1145/1067170.1067176
Siep, T. (1999). From Bluetooth to 802.15. London. Retrieved from http://grouper.ieee.org/groups/802/15/pub/1999/Jun99/99014r8P802-15_From-Bluetooth-to-802-15.ppt
Spill, D. (2012). Bluetooth Packet Sniffing Using Project Ubertooth. Ruxcon. Retrieved from http://2012.ruxcon.org.au/assets/rux/Spill-Ubertooth.pdf
Spill, D. (2013). Motivating the Problem. Retrieved August 3, 2017, from http://ubertooth.blogspot.co.uk/2013/02/motivating-problem.html
Spill, D. (2016). Unable to Sniff Pairing Requests of Bluetooth 4.0 Mobile Devices. Retrieved September 16, 2017, from https://github.com/greatscottgadgets/ubertooth/issues/201#issuecomment-223075337
Spill, D., \& Bittau, A. (2007). BlueSniff: Eve meets Alice and Bluetooth. WOOT ’07 Proceedings of the First USENIX Workshop on Offensive Technologies, 10. https://doi.org/10.1002/pssb.201300062
Tabassam, A. A., Heiss, S., \& Hoing, M. (2007). Bluetooth Device Discovery and Hop Synchronization by the Eavesdropper. In 2007 International Conference on Emerging Technologies (pp. 1–5). IEEE. https://doi.org/10.1109/ICET.2007.4516305
